Compressive sensing for dynamic spectrum access networks: Techniques and tradeoffs

We explore the practical costs and benefits of CS for dynamic spectrum access (DSA) networks. Firstly, we review several fast and practical techniques for energy detection without full reconstruction and provide theoretical guarantees. We also define practical metrics to measure the performance of these techniques. Secondly, we perform comprehensive experiments comparing the techniques on real signals captured over the air. Our results show that we can significantly compressively acquire the signal while still accurately determining spectral occupancy.

==> disc.tex <==
\section{Discussion}
\label{sec:disc}

In this paper, we have presented results that suggest compressive
sensing is a viable method for enhancing spectrum sensing for DSA
systems. Because CS allows a frontend to collect many fewer samples
than conventional ADCs, a CS-based DSA radio could sense more
spectrum with the same sampling requirements or the same spectrum with
reduced sampling requirements, resulting in cheaper and more
power-efficient systems. We have demonstrated that CS can represent
signals present in traditional whitespace spectrum, making it possible
to then detect these signals for DSA.

It is worth discussing some of the practicalities of the compressive
sensing-based hardware as opposed to a traditional Nyquist sampling
ADC receiver. As we brought up in Section~\ref{sec:intro}, there has
already been a lot of work on sub-Nyquist sampling systems for
CS~\cite{TroWakDua::2006::Random-filters,Rom::2008::Compressive-sensing,MisEld::2009::From-theory,TroLasDua::2009::Beyond-Nyquist:,DavSchSla::2010::A-wideband-compressive}. These
systems provide a distinction in how sampling rates effect the
receiver's power consumption. An ADC is composed of two main parts:
the sampling system and the comparator. It is well understood that the
majority of the ADC's power is consumed in the
comparator~\cite{le_adc2005}, and these compressive sampling hardware
systems, while they sample the signal do not require the
comparator. So the compressive sensing systems save power by both
reducing the required sampling speed and by removing the need for a
comparator.

An important point raised by the processing techniques we have used in
this study is the ability to operate on the compressed data prior to
full recovery. The recovery algorithms tend to be costly and time
consuming computations. From a time-domain perspective, DSA radios must be
able to detect and respond to changing usage patterns in a matter of
milliseconds. Also, such significant computational power required to
perform the recovery could offset the power gains achieved in the
reduction of the sampling and RF frontend. 

Unlike the analog domain, the efficiency of the digital domain grows
with Moore's law. So we can assume that digital processing of signals
will become increasingly cheaper. Currently, however, the CS
reconstruction algorithms are costly, and the simulations of the
papers we have referenced suggest large amounts of time required to
process. It has not yet been quantified what the real computational,
and therefore power, cost will be on a real DSA radio. It is important
that we have demonstrated, through off-line analysis, that reasonable
performance can be achieved by performing a coarse, instead of a full,
reconstruction.


%I really don't believe this is true.  Human made signals are VERY sparse in time-frequency, you wont do better than than Gabor.
\if 0
One of the problems with spectrum becoming less sparse is due largely to our selection of the basis
domain transform; namely, the Fourier transform. By restricting
ourselves to the frequency domain, an increase in frequency use is
problematic. Conversely, it is exactly this choice of basis domain
that has allowed us to perform signal detection on the compressed
samples without full reconstruction. However, there are other
transforms that can be explored, and other papers have presented such
approaches like the use of wavelet transforms
\cite{tian:2007:cswavelets}. This paper focused on sparse
spectrum however there is more room for analysis of this transform and the
resulting basis. It must therefore be studied if this or other domains
can be used given the timing, detection, and power requirements of DSA
radios while offering significant levels of sample compression.
\fi


==> lyric.tex <==
Compressive sensing involves sampling at a high rate, compressing the samples to a lower rate through linear mixing, and transmitting the compressed samples for further processing.  If we wish to reduce the number of evaluations of the ADC, however, we must take some care in our computation of the compressed samples.  If we simply perform an ADC on all the original samples and then compute the compressed samples with digital logic, the number of ADC evaluations (and hence the power) would remain unchanged.

Our solution to this problem has been to perform the compression in the analog domain.  Lyric Semiconductor has fabricated a chip that can perform matrix multiplication in the analog domain (in discrete time).  In particular, the signal must be sampled at the original high rate to produce a vector of continuous values, but the compression can be computed in the analog regime.  We only need to apply the ADC to the output of Lyric's chip, not the original samples.  As long as the matrix compresses the input (i.e.\ if the matrix is wider than it is tall), then we will reduce the number of ADC evaluations required.








==> results.tex <==
\section{Results}
\label{sec:results}

We first measure the...(explain metric)

\begin{figure}[htbp] %  figure placement: here, top, bottom, or page
   \centering
   \includegraphics[width=1.0\linewidth]{psd.eps} 
   \caption{A spectrogram sample of the spectrum captured around 749~MHz. These signals were sampled at 200~Msps with a 750~MHz bandpass filter.}
   \label{fig:example0}
\end{figure}
Figure~\ref{fig:example0} depicts the results of this experiment with BPDN, TV, and transpose methods depicted as solid, dashed, and dash-dotted lines, respectively.  Analysis of plot.


We next measure the...(explain metric)

\begin{figure}[htbp] %  figure placement: here, top, bottom, or page
   \centering
   \includegraphics[width=.8\linewidth]{psd.eps} 
   \caption{Here we can have another figure with the CS reconstructions, maybe a few diff examples stacked next to each other}
   \label{fig:example1}
\end{figure}
Figure~\ref{fig:example1} depicts the results of this experiment with BPDN, TV, and transpose methods depicted as solid, dashed, and dash-dotted lines, respectively.  Analysis of plot.


We next measure the...(explain metric)

\begin{figure}[htbp] %  figure placement: here, top, bottom, or page
   \centering
   \includegraphics[width=.8\linewidth]{timing1.eps} 
   \caption{Here we can have another figure with the CS reconstructions, maybe a few diff examples stacked next to each other}
   \label{fig:example2}
\end{figure}
Figure~\ref{fig:example2} depicts the results of this experiment with BPDN, TV, and transpose methods depicted as solid, dashed, and dash-dotted lines, respectively.  Analysis of plot.

\begin{figure}[htbp] %  figure placement: here, top, bottom, or page
   \centering
   \includegraphics[width=1.0\linewidth]{ff1.eps} 
   \caption{ Each reconstruction technique produces an estimate of the
     power on each channel during a period of time.  If we set our
     power threshold so that we correctly detect 90\% of the
     interferers, we waste a certain fraction of the spectrum.  This
     wasted fraction is illustrated above.}
   \label{fig:ff1}
\end{figure}

